CTTA-T: Continual Test-Time Adaptation for Text Understanding via Teacher-Student with a Domain-aware and Generalized Teacher

Text understanding often suffers from domain shifts. To handle testing domains, domain adaptation (DA) is trained to adapt to a fixed and observed testing domain; a more challenging paradigm, test-time adaptation (TTA), cannot access the testing domain during training and online adapts to the testing samples during testing, where the samples are from a fixed domain. We aim to explore a more practical and underexplored scenario, continual test-time adaptation (CTTA) for text understanding, which involves a sequence of testing (unobserved) domains in testing. Current CTTA methods struggle in reducing error accumulation over domains and enhancing generalization to handle unobserved domains: 1) Noise-filtering reduces accumulated errors but discards useful information, and 2) accumulating historical domains enhances generalization, but it is hard to achieve adaptive accumulation. In this paper, we propose a CTTA-T (continual test-time adaptation for text understanding) framework adaptable to evolving target domains: it adopts a teacher-student framework, where the teacher is domain-aware and generalized for evolving domains. To improve teacher predictions, we propose a refine-then-filter based on dropout-driven consistency, which calibrates predictions and removes unreliable guidance. For the adaptation-generalization trade-off, we construct a domain-aware teacher by dynamically accumulating cross-domain semantics via incremental PCA, which continuously tracks domain shifts. Experiments show CTTA-T excels baselines.

==> ______.tex <==
\appendix
\section{Optimality and Convergence of Asymmetric Co-Optimal Transport}
\noindent\textbf{Problem Setup and Preliminaries}

Let $\Omega_s = \{1, \dots, N\}$ and $\Omega_t = \{1, \dots, M\}$ be the index sets for samples and experts, respectively. Let $X \in \mathbb{R}^{N \times d_1}$ and $E \in \mathbb{R}^{M \times d_2}$ represent the feature matrices. The cost tensor is denoted by $L \in \mathbb{R}^{N \times M \times d_1 \times d_2}$.

We define the set of positive measures on discrete spaces as $\mathcal{M}_+(\Omega)$. The Asymmetric Co-Optimal Transport problem seeks a pair of couplings $(\pi^s, \pi^f)$ minimizing a joint cost with asymmetric marginal constraints: soft constraints on the sample side and hard constraints on the expert side.

\textbf{Definition 1 (As-COOT Objective Function)}.

The objective function $\mathcal{J}: \mathbb{R}_+^{N \times M} \times \mathbb{R}_+^{d_1 \times d_2} \to \mathbb{R} \cup \{+\infty\}$ is defined as:
\begin{equation}
\begin{aligned}
  \mathcal{J}(\pi^s, \pi^f) =& \langle L, \pi^s \otimes \pi^f \rangle + \mathcal{R}_s(\pi^s) + \mathcal{R}_f(\pi^f) \\+& \varepsilon H(\pi^s \otimes \pi^f | \mu \otimes \nu) 
  \end{aligned}
\end{equation}

where:
\begin{itemize}
    \item The coupling term is $\langle L, \pi^s \otimes \pi^f \rangle = \sum_{i,j,k,l} L_{ijkl} \pi^s_{ij} \pi^f_{kl}$.
    \item $\mathcal{R}_s(\pi^s) = \lambda_1 \text{KL}(\pi^s \mathbf{1}_M \| \mu) + \iota_{\{\mathbf{y} : \mathbf{y} = \nu\}}({\pi^s}^\top \mathbf{1}_N)$ represents the asymmetric constraint (Soft Source / Hard Target).
    \item $\mathcal{R}_f(\pi^f)$ is the analogous regularization for the feature alignment matrix.
    \item $H(\pi | \xi) = \sum \pi \log(\pi/\xi) - \pi + \xi$ is the generalized Kullback-Leibler divergence used for entropic regularization.
\end{itemize}

\noindent\textbf{Existence of Global Minimizers} 

\textit{\textbf{Theorem 1 (Existence)}} The As-COOT optimization problem admits at least one global minimizer $(\pi^s_*, \pi^f_*)$.

\textbf{Proof.} Let the feasible set be $\mathcal{F} = \{ (\pi^s, \pi^f) \in \mathbb{R}_+^{N \times M} \times \mathbb{R}_+^{d_1 \times d_2} \mid {\pi^s}^\top \mathbf{1}_N = \nu, \, {\pi^f}^\top \mathbf{1}_{d_1} = \nu_f \}$.

Compactness of Feasible Set: the constraint ${\pi^s}^\top \mathbf{1}_N = \nu$ implies that for each column $j$, $\sum_i \pi^s_{ij} = \nu_j$. Since $\pi^s_{ij} \ge 0$, each element is bounded by $0 \le \pi^s_{ij} \le \nu_j$. Thus, $\pi^s$ belongs to a closed and bounded subset of Euclidean space, which is compact by the Heine-Borel theorem. The same applies to $\pi^f$. Therefore, the product space $\mathcal{F}$ is compact.

Lower Semi-Continuity (L.S.C.):
\begin{itemize}
    \item The bilinear term $\langle L, \pi^s \otimes \pi^f \rangle$ is continuous w.r.t. $(\pi^s, \pi^f)$.
    \item The KL divergence is continuous on its domain and strictly convex.
    \item The indicator function $\iota_{\{\cdot=\nu\}}$ is L.S.C. (it is the convex indicator of a closed set).
    \item The sum of L.S.C. functions is L.S.C.
\end{itemize}
By the Weierstrass Extreme Value Theorem, a lower semi-continuous function on a non-empty compact set attains its minimum.


\noindent\textbf{Sub-problem Analysis: Convexity and Duality}

Since the objective is non-convex jointly but bi-convex, we analyze the sub-problem where one variable is fixed. Without loss of generality, fix $\pi^f$ and let $C^s_{ij} = \sum_{k,l} L_{ijkl} \pi^f_{kl}$.

Problem $\mathcal{P}_s(\pi^f)$:
\begin{equation}
    \begin{aligned}
        \min_{\pi^s \ge 0} \quad& \langle C^s, \pi^s \rangle + \lambda_1 \text{KL}(\pi^s \mathbf{1}_M \| \mu) \\+& \iota_{\{\nu\}}({\pi^s}^\top \mathbf{1}_N) + \varepsilon \text{KL}(\pi^s \| \mu \otimes \nu)
    \end{aligned}
\end{equation}

\textbf{Strict Convexity.} Problem $\mathcal{P}_s(\pi^f)$ is strictly convex w.r.t $\pi^s$.

\textbf{Proof.} The term $\varepsilon \text{KL}(\pi^s \| \mu \otimes \nu)$ involves the function $x \log x$, which has a positive second derivative ($1/x > 0$ for $x>0$). The linear terms and the indicator function are convex. The sum of a strictly convex function and convex functions is strictly convex. Thus, if a solution exists, it is unique. 

\textbf{Fenchel-Rockafellar Dual Derivation.}
To derive the optimal update law, we construct the Lagrangian dual.Let $g(\pi^s) = \lambda_1 \text{KL}(\pi^s \mathbf{1}_M \| \mu)$ and $h(\pi^s) = \iota_{\{\nu\}}({\pi^s}^\top \mathbf{1}_N)$.The primal problem is:
\begin{equation}
    \min_{\pi^s} \mathcal{E}(\pi^s) + g(A\pi^s) + h(B\pi^s)
\end{equation}
where $\mathcal{E}$ is the entropic cost, $A$ sums rows, and $B$ sums columns.

Using Fenchel duality, the dual problem is:
\begin{equation}
    \begin{aligned}
            \max_{\alpha \in \mathbb{R}^N, \beta \in \mathbb{R}^M}& - g^*(-\alpha) - h^*(-\beta) \\&- \varepsilon \sum_{i,j} \exp\left( \frac{\alpha_i + \beta_j - C^s_{ij}}{\varepsilon} \right)
    \end{aligned}
\end{equation}

where $g^*$ and $h^*$ are the Legendre-Fenchel conjugates:
\begin{itemize}
    \item Soft Constraint Conjugate ($g^*$): For $g(x) = \lambda_1 \sum (x_i \log(x_i/\mu_i) - x_i + \mu_i)$, the conjugate is:
    \begin{equation}
        g^*(y) = \lambda_1 \sum_i \mu_i \left( e^{y_i/\lambda_1} - 1 \right)
    \end{equation}

    \item Hard Constraint Conjugate ($h^*$): For $h(x) = \iota_{\{\nu\}}(x)$, the conjugate is linear:
    \begin{equation}
    h^*(y) = \langle y, \nu \rangle
    \end{equation}
\end{itemize}

Substituting these into the dual objective:
\begin{equation}
\begin{aligned}
        \max_{\alpha, \beta} &-\lambda_1 \sum_i \mu_i \left( e^{-\alpha_i/\lambda_1} - 1 \right) + \langle \beta, \nu \rangle \\&- \varepsilon \sum_{i,j} \mu_i \nu_j e^{(\alpha_i + \beta_j - C^s_{ij})/\varepsilon}
\end{aligned}
\end{equation}


\noindent\textbf{Optimality Conditions (KKT).}
Setting the gradient of the dual objective w.r.t $\alpha_i$ and $\beta_j$ to zero yields the optimality conditions.

For $\alpha_i$:
\begin{equation}
    \mu_i e^{-\alpha_i/\lambda_1} = \sum_j \mu_i \nu_j e^{(\alpha_i + \beta_j - C^s_{ij})/\varepsilon}
\end{equation}
\begin{equation}
    e^{-\alpha_i/\lambda_1} = e^{\alpha_i/\varepsilon} \sum_j K_{ij} e^{\beta_j/\varepsilon} \quad 
\end{equation}
where $K_{ij} = e^{-C^s_{ij}/\varepsilon}$

Let $u_i = e^{\alpha_i/\varepsilon}$ and $v_j = e^{\beta_j/\varepsilon}$. The equation becomes:
\begin{equation}
    u_i^{-\varepsilon/\lambda_1} = u_i \sum_j K_{ij} \nu_j v_j
\end{equation}


Rearranging for $u_i$:
\begin{equation}
u_i = \left( \sum_j K_{ij} \nu_j v_j \right)^{-\frac{\lambda_1}{\lambda_1 + \varepsilon}}
\end{equation}


For $\beta_j$ (Hard constraint):
\begin{equation}
\nu_j = \sum_i \mu_i \nu_j e^{(\alpha_i + \beta_j - C^s_{ij})/\varepsilon}
\end{equation}
\begin{equation}
1 = v_j \sum_i u_i K_{ij} \mu_i \implies v_j = \frac{1}{\sum_i \mu_i K_{ij} u_i}
\end{equation}

\textbf{\textit{Theorem 2 (Optimal Sub-problem Solution)}}

The unique global minimizer $\pi^s_*$ for the fixed-$\pi^f$ sub-problem is given by:
\begin{equation}
    \pi^s_{ij} = u_i K_{ij} v_j \mu_i \nu_j
\end{equation}

where vectors $u$ and $v$ are determined by the fixed-point iterations of the generalized Sinkhorn algorithm derived above.

\noindent\textbf{Convergence of Block Coordinate Descent (BCD)}

The As-COOT algorithm alternates between solving for $\pi^s$ and $\pi^f$. We model this as a Block Coordinate Descent on the objective $\mathcal{J}$.

Algorithm Flow:

$\pi^s_{k+1} = \arg\min_{\pi^s} \mathcal{J}(\pi^s, \pi^f_k)$

$\pi^f_{k+1} = \arg\min_{\pi^f} \mathcal{J}(\pi^s_{k+1}, \pi^f)$

\textbf{\textit{Theorem 3 (Monotonicity and Convergence)}}
The sequence $\{(\pi^s_k, \pi^f_k)\}_{k \in \mathbb{N}}$ generated by As-COOT satisfies. Monotonicity: $\mathcal{J}(\pi^s_{k+1}, \pi^f_{k+1}) \le \mathcal{J}(\pi^s_k, \pi^f_k)$. Stationarity: Every limit point of the sequence is a stationary point of the problem.

\textbf{Proof.} 

Descent Property: by definition of the update steps:
\begin{equation}
    \mathcal{J}(\pi^s_{k+1}, \pi^f_k) \le \mathcal{J}(\pi^s_k, \pi^f_k) 
\end{equation}
since $\pi^s_{k+1}$ is the global minimizer
\begin{equation}
\mathcal{J}(\pi^s_{k+1}, \pi^f_{k+1}) \le \mathcal{J}(\pi^s_{k+1}, \pi^f_k) 
\end{equation}
since $\pi^f_{k+1}$ is the global minimizer

Summing these inequalities confirms $\mathcal{J}_{k+1} \le \mathcal{J}_k$. Since $\mathcal{J}$ is bounded below (by 0), the sequence of objective values converges.

Convergence to Stationary Point: the objective function $\mathcal{J}$ can be decomposed as:
\begin{equation}
    \mathcal{J}(\pi^s, \pi^f) = f(\pi^s, \pi^f) + \sum_i g_i(\pi^s) + \sum_j h_j(\pi^f)
\end{equation}

where $f$ is the smooth differentiable part (coupling term + entropic parts treated smoothly in the interior) and $g, h$ are the non-smooth convex indicator functions for constraints.

According to Tseng's Theorem \cite{} on Coordinate Descent for non-smooth separable functions:
\begin{itemize}
    \item The non-smooth parts are separable (indicator on $\pi^s$ does not depend on $\pi^f$).
    \item The smooth part is regular on the domain.
    \item The sub-problems maximize a strictly concave dual (or minimize a strictly convex primal) and have unique solutions.
\end{itemize}

Under these conditions, any limit point $(\bar{\pi}^s, \bar{\pi}^f)$ of the sequence satisfies the first-order optimality conditions (stationary point):
\begin{equation}
    0 \in \partial_{\pi^s} \mathcal{J}(\bar{\pi}^s, \bar{\pi}^f) \quad \text{and} \quad 0 \in \partial_{\pi^f} \mathcal{J}(\bar{\pi}^s, \bar{\pi}^f)
\end{equation}
Thus, As-COOT converges to a coordinate-wise minimum.

We have rigorously established the following properties for As-COOT. (1) Well-Posedness: The problem is defined on a compact set with a lower semi-continuous objective, guaranteeing the existence of an optimal solution (\textit{Theorem 1}). (2) Tractability: The non-convex joint problem decomposes into strictly convex sub-problems. Through Fenchel duality, we proved that the sub-problems admit a unique solution expressible via efficient generalized Sinkhorn scalings (\textit{Theorem 2}). (3) Algorithmic Convergence: The Block Coordinate Descent strategy is theoretically guaranteed to monotonically decrease the objective and converge to a stationary point (\textit{Theorem 3}).

This theoretical foundation confirms that As-COOT is not merely a heuristic, but a mathematically sound optimization framework for asymmetric distribution alignment.

==> tables/IPCA_table.tex <==
\begin{table}[htbp]
    \caption{Performance of our method and models with four fixed EMA weights on Orders 1 – 6. \textbf{Bold}: best results.}
    \label{tab:ipca}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccccc|cccccc|cc}
        \toprule
        \multicolumn{1}{l}{} & \multicolumn{6}{c}{\textbf{Short Sequence}} & \multicolumn{6}{c}{\textbf{Long Sequence}} &  \\
        \midrule
          \multicolumn{1}{l}{\textbf{Time}}& \multicolumn{2}{c}{\textbf{t}$\longrightarrow$} & \multicolumn{2}{c}{\textbf{t}$\longrightarrow$} & \multicolumn{2}{c}{\textbf{t}$\longrightarrow$} & \multicolumn{2}{c}{\textbf{t}$\longrightarrow$} & \multicolumn{2}{c}{\textbf{t}$\longrightarrow$} & \multicolumn{2}{c}{\textbf{t}$\longrightarrow$} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Avg}}} \\
         \textbf{Order}& \multicolumn{2}{c}{\textbf{Order1}} & \multicolumn{2}{c}{\textbf{Order2}} & \multicolumn{2}{c|}{\textbf{Order3}} & \multicolumn{2}{c}{\textbf{Order4}} & \multicolumn{2}{c}{\textbf{Order5}} & \multicolumn{2}{c|}{\textbf{Order6}} &  \\
        \midrule
        Methods & EM & F1 & EM & F1 & EM & F1 & EM & F1 & EM & F1 & EM & F1 & EM & F1 \\
        \midrule
        CTTA-T (ours) & \textbf{54.14} & \textbf{66.57} & \textbf{53.88} & \textbf{66.01} & \textbf{54.07} & \textbf{66.12} & \textbf{57.74} & \textbf{69.33} & \textbf{57.63} & \textbf{69.33} & \textbf{57.71} & \textbf{69.24} & \textbf{55.86} & \textbf{67.77} \\
        $\alpha=1.00$ & 54.04 & 66.12 & 53.69 & 65.97 & 53.89 & 66.03 & 57.49 & 69.15 & 57.23 & 68.98 & 57.38 & 69.07 & 55.62 & 67.55 \\
        $\alpha=0.99$ & 53.51 & 65.83 & 53.40 & 65.55 & 53.14 & 65.40 & 57.30 & 68.86 & 57.43 & 68.95 & 57.36 & 68.83 & 55.36 & 67.24 \\
        $\alpha=0.50$ & 38.96 & 50.13 & 39.47 & 49.68 & 46.17 & 55.85 & 39.52 & 48.15 & 8.23 & 14.65 & 32.27 & 41.70 & 34.10 & 43.36 \\
        $\alpha=0$ & 42.38 & 53.10 & 36.47 & 45.96 & 49.56 & 60.56 & 37.74 & 45.30 & 22.82 & 30.31 & 12.49 & 15.57 & 33.58 & 41.80 \\
        \bottomrule
    \end{tabular}
    }
\end{table}

